Implicit Multiagent Coordination at Unsignalized Intersections via Multimodal Inference Enabled by Topological Braids

We focus on navigation among rational, non-communicating agents at unsignalized street intersections. Following collision-free motion under such settings demands nuanced implicit coordination among agents. Often, the structure of these domains constrains multiagent trajectories to belong to a finite set of modes. Our key insight is that empowering agents with a model of these modes can enable effective coordination, realized implicitly via intent signals encoded in agents' actions. In this paper, we represent modes of joint behavior in a compact and interpretable fashion using the formalism of topological braids. We design a decentralized planning algorithm that generates actions aimed at reducing the uncertainty over the mode of the emerging multiagent behavior. This mechanism enables agents that individually run our algorithm to collectively reject unsafe intersection crossings. We validate our approach in a simulated case study featuring challenging multiagent scenarios at a four-way unsignalized intersection. Our model is shown to reduce frequency of collisions by >65% over a set of baselines explicitly reasoning over trajectories, while maintaining comparable time efficiency.

==> sections/bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/mavrogiannis}}]{Christoforos Mavrogiannis}
(S’ 12–M’ 19) received a diploma in mechanical engineering from the National Technical University of Athens, Greece in 2013, and the M.S. and Ph.D. degrees from Cornell University in 2017 and 2019, respectively. 

He is currently a postdoctoral research associate in the Paul G. Allen School of Computer Science \& Engineering at the University of Washington, Seattle. His research interests include multiagent systems, human-robot interaction, and robotic manipulation.


\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/decastro}}]{Jonathan A. DeCastro} (S'12--M'17) received the B.S. and M.S. degrees in mechanical engineering from Virginia Tech in 2001 and 2003, respectively and the M.S. and Ph.D. degrees from Cornell University in 2014 and 2017, respectively. 

He is currently a Research Scientist at the Toyota Research Institute in Cambridge, MA.  His current research interests include formal verification, provable testing strategies, interpretable agent behavior modeling, and applications to robot planning and control.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/srinivasa}}]{Siddhartha S. Srinivasa} (S’02–M’08–SM’16– F’18) received the B.Tech. degree in mechanical engineering from the Indian Institute of Technology Madras, Chennai, India, in 1999 and the Ph.D. degree in robotics from Carnegie Mellon University, Pittsburgh, Pennsylvania, in 2005. He is the Boeing Endowed Professor at the School of Computer Science \& Engineering, University of Washington, Seattle, WA, USA. He works on robotic manipulation, with the goal of enabling robots to perform complex manipulation tasks under uncertainty and clutter, with and around people. To this end, he founded the Personal Robotics Lab in 2005. He is also passionate about building end-to-end systems (HERB, ADA, HRP3, CHIMP, Andy, among others) that integrate perception, planning, and control in the real world. Understanding the interplay between system components has helped produce state-of-the-art algorithms for robotic manipulation, motion planning, object recognition, and pose estimation (MOPED), dense 3-D modeling (CHISEL, now used by Google Project Tango), and mathematical models for human–robot collaboration.
\end{IEEEbiography}
